Small Forcing Makes Any Cardinal Superdestructible

Small forcing always ruins the indestructibility of an indestructible supercompact cardinal. In fact, after small forcing, any cardinal $\kappa$ becomes superdestructible---any further ${<}\kappa$-closed forcing which adds a subset to $\kappa$ will destroy the measurability, even the weak compactness, of $\kappa$. Nevertheless, after small forcing indestructible cardinals remain resurrectible, but never strongly resurrectible.

==> arrowmacros.tex <==
\font\arrow=line10 scaled \magstep1
\def\makeline#1.{\hbox{\arrow\char#1}}
\def\makearrow#1.#2.{\hbox{\arrow\char#1\llap{\char#2}}}
\def\definelinesandarrows#1.#2.#3.#4.#5.{
   \expandafter\edef\csname#4line\endcsname{\makeline#1.}
   \expandafter\edef\csname#4arrow\endcsname{\makearrow#1.#2.}
   \expandafter\edef\csname#5line\endcsname{\makeline#1.}
   \expandafter\edef\csname#5arrow\endcsname{\makearrow#1.#3.}}
\definelinesandarrows 0.18.9.ne.sw.
\definelinesandarrows 1.21.11.nnne.sssw.
\definelinesandarrows 2.14.13.nnnne.ssssw.
\definelinesandarrows 3.23.15.nnnnne.sssssw.
\definelinesandarrows 4.23.15.nnnnnne.ssssssw.
\definelinesandarrows 10.30.29.nne.ssw.
\definelinesandarrows 16.49.41.neeeeee.swwwwww.
\definelinesandarrows 17.51.43.neeee.swwww.
\definelinesandarrows 19.55.47.nehuh.swhuh.
\definelinesandarrows 24.58.41.neeeeeee.swwwwwww.
\definelinesandarrows 26.62.9.neee.swww.
\definelinesandarrows 33.49.25.neeeee.swwwww.
\definelinesandarrows 35.62.61.nee.sww.
\definelinesandarrows 64.82.73.se.nw.
\definelinesandarrows 65.85.75.ssse.nnnw.
\definelinesandarrows 66.78.77.sssse.nnnnw.
\definelinesandarrows 67.87.79.ssssse.nnnnnw.
\definelinesandarrows 68.87.79.sssssse.nnnnnnw.
\definelinesandarrows 74.94.93.sse.nnw.
\definelinesandarrows 80.113.105.seeeeee.nwwwwww.
\definelinesandarrows 81.115.107.seeee.nwwww.
\definelinesandarrows 99.126.125.see.nww.
\def\sejoin#1#2{\setbox1=\hbox{#1}\setbox2=\hbox{#2}%
  \hbox{\vbox{\hbox{\copy1\kern\wd2}\nointerlineskip
              \hbox{\kern\wd1\box2}}}}
\def\nejoin#1#2{\setbox1=\hbox{#1}\setbox2=\hbox{#2}%
  \hbox{\vbox{\hbox{\kern\wd1\copy2}\nointerlineskip\hbox{\copy1\kern\wd2}}}}
\newdimen\hnudge
\newdimen\vnudge
\newdimen\hnudgedefault
\newdimen\vnudgedefault
\def\NEdefaultnudge{\hnudge=-16pt\vnudge=16pt}
\def\SEdefaultnudge{\hnudge=-16pt\vnudge=20pt}
\def\Edefaultnudge{\hnudge=-25pt\vnudge=6pt}
\def\Sdefaultnudge{\hnudge=-8pt\vnudge=20pt}
\def\longEdefaultnudge{\hnudge=-5pt\vnudge=6pt}
\def\nudgeright#1pt{\advance\hnudge by#1pt}
\def\nudgeleft#1pt{\advance\hnudge by-#1pt}
\def\nudgeup#1pt{\advance\vnudge by#1pt}
\def\nudgedown#1pt{\advance\vnudge by-#1pt}
\def\label#1{\smash{\llap{\kern\hnudge
                   \raise\vnudge\rlap{$\scriptstyle#1$}\hfill}}}
\def\NEarrow{\NEdefaultnudge
             \nejoin\neeline{\nejoin\neeline{\nejoin\neeline\neearrow}}}
\def\SWarrow{\NEdefaultnudge
             \nejoin\swwarrow{\nejoin\swwline{\nejoin\swwline\swwline}}}
\def\SEarrow{\SEdefaultnudge
             \sejoin\seeline{\sejoin\seeline{\sejoin\seeline\seearrow}}}
\def\NWarrow{\SEdefaultnudge
             \sejoin\nwwarrow{\sejoin\nwwline{\sejoin\nwwline\nwwline}}}
\def\Sarrow{\Sdefaultnudge\setbox1=\hbox{\SEarrow}
           \hbox{\hskip 10pt\vrule height\ht1\hbox{\arrow\char'77}}}
\def\Earrow{\Edefaultnudge\setbox1=\hbox{\SEarrow}
 \hbox{\raise 2pt\hbox{\vrule height-.4pt depth.8ptwidth\wd1\kern2pt
       \llap{\arrow\char'55}}}}
\def\longEarrow{\longEdefaultnudge\setbox1=\hbox{\SEarrow}
      \rlap{\hskip-1.25\wd1\raise 2pt
            \hbox{\vrule height-.4pt depth.8ptwidth2.5\wd1\kern2pt
            \llap{\arrow\char'55}}}}
\def\trianglediagram#1#2#3#4#5#6{%
    {\def\normalbaselines{\baselineskip0pt\lineskip8pt\lineskiplimit0pt}%
       \matrix{#1& &\cr
               \Sarrow\label{#2}&\SEarrow\label{#3}&\cr
               #4&\Earrow\label{#5}&#6\cr}}}
\def\extenddiagram#1#2#3#4#5#6#7#8#9{%
     {\def\normalbaselines{\baselineskip0pt\lineskip8pt\lineskiplimit0pt}%
        \matrix{#1 & \of & #2 & & \cr
               \Sarrow\label{#3}&\SEarrow\label{#4}& &\SEarrow\label{#5}&\cr
               #6&\Earrow\label{#7}&#8&\of&#9\cr}}}

